Inverse Diffusion Curves using Shape Optimization

The inverse diffusion curve problem focuses on automatic creation of diffusion curve images that resemble user provided color fields. This problem is challenging since the 1D curves have a nonlinear and global impact on resulting color fields via a partial differential equation (PDE). We introduce a new approach complementary to previous methods by optimizing curve geometry. In particular, we propose a novel iterative algorithm based on the theory of shape derivatives. The resulting diffusion curves are clean and well-shaped, and the final image closely approximates the input. Our method provides a user-controlled parameter to regularize curve complexity, and generalizes to handle input color fields represented in a variety of formats.

==> introduction.tex <==
\section{Introduction}
% -> popularity of DC

Vector graphic images are widely used in computer graphics. Their compact representation offers many
advantages, notably scalability and editability. 
The recently developed diffusion curve images~\cite{Orzan:2008} have further
improved the expressiveness of vector graphics.
By diffusing colors defined along a set of curves, these images can represent rich color distributions and  depict complex
geometry and shading effects.
%
%These advantages have made them a popular tool for graphic designers
%and triggered n
Numerous efforts have further improved their performance, extended 
expressiveness, and developed novel applications
(e.g.,~\cite{Jeschke:2009,TSNI10,Sun:2012:DCT,Ilbery:2013:BDC,Sun:2014:FMR}).

Despite the conceptual simplicity of diffusion curve images, creating them
automatically (given desired target images) is  difficult.
This is because 1D diffusion curves yield resulting 2D color fields via
a partial differential equation (PDE). Local changes of the curve
geometry have a global and complex impact on the color values over a
whole 2D region. This makes the inverse problem of finding diffusion curves that best approximate an input image extremely hard. 
Instead, previous methods rely on a common \emph{heuristic} of placing curves along images'
discontinuous ``edges'' detected locally from the image
gradient~\cite{Orzan:2008} or Laplacian (and/or bi-Laplacian)
domain~\cite{Xie:2014:HDC}.
This makes it hard to handle smooth regions where no edge is present but where color varies enough.
%
\begin{comment}
    To tackle this challenge, a key question one needs to answer is where to place diffusion curves.
    Indeed, this question has been investigated since the invention of diffusion curve images, in the context of pixel image vectorization~\cite{Orzan:2008,Xie:2014:HDC}.
    % -> vectorization -> edge detection -> incompletely
    These methods %place diffusion curves based on a common observation: a diffusion curve color field is continuous everywhere except on the curves.
    %Thus, they place curves along images' discontinuous ``edges'', whether they are detected from the image gradient~\cite{Orzan:2008} or Laplacian (and/or bi-Laplacian) domain~\cite{Xie:2014:HDC}.
    share a common \emph{heuristic} of placing curves along images' discontinuous ``edges''
    detected locally from the image gradient~\cite{Orzan:2008} or Laplacian (and/or
    bi-Laplacian) domain~\cite{Xie:2014:HDC}.
    In a sufficiently continuous color region, however, no curve is placed. 
    Rather, such a region is approximated using a harmonic and/or biharmonic color function,
    although its true color variation can be much more complex. % than a harmonic or biharmonic function.  
    These methods perform well at image edges but can have difficulty handling smoothly colored regions
    where well-defined edges are hard to find but where variations are strong enough to require curves.
\end{comment}

\begin{comment}
    In a sufficiently continuous color region, however, edge detection methods can
    fail to find any edges even in a high-order derivative domain, and thus no
    curve is placed there. Rather, such a region is approximated using a harmonic
    and/or biharmonic color function.
    
    Clearly, a region with continuous colors can be much more complex than a
    harmonic or biharmonic function.  For instance, according to the classical
    maximum principle, both harmonic and biharmonic function can have local maxima
    \emph{only} on the boundary, fundamentally limiting their ability to
    approximate a color region whose local maxima is located inside
    (Figure~\todo{F}).
\end{comment}

% new approach: place curves in smooth region --> where to place: hard --> move curves + optimization
We propose a complementary yet fundamentally novel approach for the automated
placement of diffusion curves in complex smooth image regions.
\begin{comment}
    In addition to fixing curves at \sz{color discontinuities (i.e., edges)}, our method
    %, complementary to all previous approaches, 
    is focused on the problem of generating curves in regions of \emph{continuous} colors. 
    % -> where to place 
    Through the optimization of curve geometries and topologies \szrem{do we need to mention ``topologies''?}, we develop an algorithm that produces diffusion curves to closely represent a provided color field,
    and meanwhile keeps the curves well-shaped and clean.
\end{comment}
Unlike existing methods that rely on local heuristics, our method places diffusion curves through \emph{global optimization} of curve geometry, taking into account the global impact of a curve on the final color field. 
This results in well shaped curves that accurately reproduce the input image, even in complex smooth regions. We focus on complex smooth regions, and use standard approaches for discontinuities. 

%
%The resulting curves are well-shaped and clean, and the final image closely represents the provided color field.
%In particular, w

We formulate the diffusion curve placement as a \emph{shape optimization} problem constrained by a PDE 
(i.e., Laplace's equation).
Given a color field, our method generates curves to minimize a measure of the color approximation residual. %subject to the Laplace's equation for color diffusion.
Starting from an initial set of curves, it iteratively evolves their shapes (and possibly topologies) toward an optimal placement.
Mathematically, the curves are treated as continuous functionals.
This allows the curves to deform %almost
arbitrarily, enabling full exploration of possible placements.
This iterative process is similar to a surface normal flow:
our curve evolution at every iteration is guided by the \FC derivative of the residual function with respect to the curve's surface velocity, leading to an efficient ``gradient descent'' of the residual.
This method enjoys mathematical elegance: all computations at each iteration boil down to numerically solving a Laplace's equation and a Poisson's equation.
Leveraging existing software libraries, it is also easy to implement.

% => advantages
Building on our curve placement algorithm, we introduce a complete pipeline
for automatic generation of diffusion curve images.
Our method is able to place high-quality diffusion curves in a clean and
concise way, and generate diffusion curve images closely
representing complex color variations of the reference color field (Figure~\ref{fig:teaser}).
Our method also allows the user to trade approximation accuracy for curve
simplicity, a desired feature for retaining vector graphics' editability.
%Extensions controlling color variations on resulting curves are also possible.
\begin{comment}
    In addition, the efficacy of our optimized curves in turn eases the edge
    detection methods: we only need to fix a few curves along contour edges
    detected on the original color field---not even in the gradient domain. Thus,
    the resulting curves become simpler and cleaner, as detecting edges in
    higher-order domains is more prone to color noise and can result in a region of
    ``edge soup'' (Figure~\todo{f}).
\end{comment}
In addition, our approach (which focuses on continuously colored regions) is
complementary to existing edge-detection-based methods (which seek for
discontinuities) and can be used together with them.
Lastly, our method utilizes the per-pixel blurring feature originally introduced
in~\cite{Orzan:2008}, which has been ignored by existing image
vectorization methods, during post-processing.

% => not necessarily a pixel images
% => clean and less curves
% => side effect: no need to conduct in high-order derivative domain

%Building on our curve placement algorithm, we obtain a complete pipeline for automatic generation of diffusion curve images.
We validate the quality of resulting images by comparing with ground-truth
color fields using a numerical error metric as well as a calibrated visual
metric.


==> makefile <==
# name of latex document
MAINDOC := curveopt_arxiv

# latex source file
TEXSRC := curveopt_arxiv.tex diff_curve_opt.tex motivation.tex curve_gen.tex introduction1.tex conclusion.tex results.tex abstract.tex related.tex appendix.tex
BIBSRC := $(wildcard *.bib)

ifneq ($(strip $(BIBSRC)),)
BBLSRC := $(MAINDOC).bbl
endif

# latex program
TEX      := latex
PDFLATEX := pdflatex
BIB      := bibtex

# flags
TEX_FLAGS :=
PDF_FLAGS :=
BIB_FLAGS :=

#=====================================================#
# Display Codes (this is so we can track passes)
#=====================================================#
MOVE_TO_COL	= @echo  "\\033[60G"
SETCOLOR_RED 	= @echo  "\\033[0;31m"
SETCOLOR_GREEN 	= @echo  "\\033[0;32m"
SETCOLOR_BLUE	= @echo  "\\033[0;34m"
SETCOLOR_BACK	= @echo  "\\033[0m"

all: $(MAINDOC).pdf

pdf: $(MAINDOC).pdf

dvi: $(MAINDOC).dvi

full: $(BBLSRC) $(TEXSRC)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================FINAL PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)


%.dvi : %.aux
	$(SETCOLOR_BLUE)
	@echo "=========================AUX -> DVI PASS=============================="
	$(SETCOLOR_BACK)
	@$(TEX) $(TEX_FLAGS) $(*F)
	
$(MAINDOC).bbl : $(BIBSRC) $(TEXSRC) 
ifneq ($(strip $(BIBSRC)),)
	$(SETCOLOR_GREEN)
	@echo "=========================LaTeX PASS=============================="
	$(SETCOLOR_BACK)
	$(PDFLATEX) $(TEX_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================BibTex PASS=============================="
	$(SETCOLOR_BACK)
	@$(BIB) $(BIB_FLAGS) $(MAINDOC)
endif

$(MAINDOC).pdf : $(TEXSRC)
	$(SETCOLOR_GREEN)
	@echo "=========================SINGLE PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)

.PHONY: all clean

clean:
	-$(RM) *.aux *.pdf *.bbl *.blg *.log

